Tuning Confidence Bound for Stochastic Bandits with Bandit Distance

We propose a novel modification of the standard upper confidence bound (UCB) method for the stochastic multi-armed bandit (MAB) problem which tunes the confidence bound of a given bandit based on its distance to others. Our UCB distance tuning (UCB-DT) formulation enables improved performance as measured by expected regret by preventing the MAB algorithm from focusing on non-optimal bandits which is a well-known deficiency of standard UCB. "Distance tuning" of the standard UCB is done using a proposed distance measure, which we call bandit distance, that is parameterizable and which therefore can be optimized to control the transition rate from exploration to exploitation based on problem requirements. We empirically demonstrate increased performance of UCB-DT versus many existing state-of-the-art methods which use the UCB formulation for the MAB problem. Our contribution also includes the development of a conceptual tool called the "Exploration Bargain Point" which gives insights into the tradeoffs between exploration and exploitation. We argue that the Exploration Bargain Point provides an intuitive perspective that is useful for comparatively analyzing the performance of UCB-based methods.

==> include.backup0920/author.tex <==

\hypersetup{
	pdftitle={Tuning Confidence Bound for Stochastic Bandits with Bandit Distance},
	pdfsubject={statistics},
	pdfauthor={Xinyu Zhang},
	pdfkeywords={Multi-Armed Bandits, UCB, Confidence Bound},
	}

	
\title{Tuning Confidence Bound for Stochastic Bandits with Bandit Distance}


\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@eng.ucsd.edu}
	\And
	Srinjoy Das\\
	West Virginia University\\
	\texttt{srinjoy.das@mail.wvu.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@eng.ucsd.edu} 
}


==> include.backup0920/body.tex <==

\begin{abstract}
	We discover a novel modification upon the standard UCB method, which tunes
	confidence bound using bandit distance. Our formulation is simple to
	understand, straightforward for bound analysis, extensible, and naturally
	models the transition from exploration to exploitation. Our proposed
	distance measure can be customized to control the transition speed. We
	empirically demonstrate its strong performance over many latest methods.
	Along with the analysis of our method, we propose a new concept called
	\textit{Exploration Bargain Point} to intuitively explain why under
	exploration can be beneficial for upper confidence bound methods.
																																																																																																																																																																																																							
\end{abstract}


\section{Introduction}


Multi-armed bandit (MAB) problem \cite{slivkins_tutorial} can model a broad
range of applications, such as selecting the best website layout for users, or
choosing the most profitable stocks among many. Stochastic bandits is the
fundamental model of MAB, and one of the most influential and widely used
stochastic bandit policy is upper confidence bound method (UCB)
\cite{auer2002finite}. UCB works by maintaining a mean estimation and confidence
radius\footnote{We will refer confidence radius as confidence bound in the rest
of the paper.} for each bandit, and selecting the bandit with maximum sum of
mean and confidence bound at each step. The confidence bound can grow larger for
less-frequently used bandits which represents a higher degree of uncertainty to
serve the exploration purpose.


% However, UCB could waste many trials on non-optimal bandits by being optimistic
% indiscriminately. 

However, UCB by nature leads to unsatisfactory results  by being
over-optimistic on non-optimal bandits. In this work, we propose a simple
modification to the original UCB method which makes the confidence bound of one
bandit depends on its distance to others. Since the policy will select the
largest bandit more often, so the exploration will naturally lean towards the
neighbor of the largest bandit and save attempts from bad ones. An example is
provided in Fig. \ref{fig:intro}.


\begin{figure}[h]
	\vspace*{-8pt}
	\centering
	\scalebox{0.30}{
		\input{plots/pgf/intro_graph.pgf}
	}
	\vspace*{-8pt}
	\caption{Confidence bound comparison to UCB in a two-arm Bernoulli setting. By
	tunning confidence bound, the policy attempts fewer on the non-optimal one.}
	\label{fig:intro}
\end{figure}



By introducing bandit distance, we offer the opportunity of customization over policies
through different distances. Therefore, our formulation can represent a family of policies
which inherently model the transition from pro-exploration policy, such as UCB, to
pro-exploitation policy like greedy.


Moreover, many existing methods, including ours, redesign confidence bound to
under-explore than UCB. An interesting question can be asked: What is the drawback of using
the standard confidence bound if it is derived from the well-established concentration
inequality? 
Previous methods answer this implicitly by proving stricter 
regret bound. However, they are are neither straightforward nor intuitive
enough, while intuition undoubtedly can help us to gain deeper understanding and
improve a system. In this
paper, we present a novel concept named \textit{Exploration Bargain
Point} to answer this question directly and even graphically from a new
perspective. 



There are many existing work about the design of confidence bound, which we
will discuss in Sec. \ref{sec:relate}. While having connections to these
previous successive approaches, we make the following contributions in this paper.


\begin{itemize}
	\item We propose a new UCB-based policy, which tunes confidence bound by
	      bandit distance. We conduct analysis and numerical experiments to show our
	      formulation is simple, extensible, and performant.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
	\item We present a novel concept called \textit{Exploration Bargain Point},
	      which provides a new viewpoint of analysis on why exploration should
	      early stop in the context of upper confidence bound methods.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
\end{itemize}


\section{Preliminaries}



Let $k \in \mathbb{Z}^+$ be the number of bandits, $T$ denote the time horizon,
$\mu_i \in \mathbb{R}$ be the unknown mean for the distribution of bandit $i$,
$\mu_* = \max_i \mu_i$ be the mean of the optimal bandit, $B_i$ be the shorthand
for \quotes{bandit $i$} where $i\in[k]$. In each round $t \in [T] = \{1,2,...,T\}$, the policy
chooses a bandit $A_t \in [k]$ and receives an observation denoted by random
variable $X_t$.



We use $\Delta_i = \mu_* - \mu_i$ to represent the suboptimality gap for $i$th
bandit, and $N_i(t)$ to represent the number of times bandit $i$ gets chosen till $t$.
The regret over $T$ rounds is

\begin{equation}
	\mathcal{R}_{T}=\sum_{i=1}^k \Delta_{i} \mathbb{E}\left[N_{i}(T)\right]
	\label{eq:regret}
\end{equation}

which serves as the main metric for stochastic bandit policies. A policy is
called \textit{asymptotically optimal} if

$$
\lim _{T \rightarrow \infty} \frac{\mathcal{R}_{T}}{\log (T)}=\sum_{i: \Delta_{i}>0} \frac{2}{\Delta_{i}}
$$

\cite{lai1985asymptotically,burnetas1997optimal} show that the above forms a
regret upper bound for all consistent policies. A policy is called
\textit{sub-UCB} \cite{lattimore2018refining}, which is a stricter requirement
than \textit{asymptotically optimality}, if there exists universal constants
$C_1, C_2 > 0$, the regret can be finitely bounded as

$$
\mathcal{R}_{t} \leq C_{1} \sum_{i=1}^{k} \Delta_{i} + C_{2} \sum_{i: \Delta_{i}(\mu)>0} \frac{\log (n)}{\Delta_{i}}
$$


The UCB policy works by choosing bandit $A_t$ that

$$
A_t = \arg\max_{i \in [k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{N_i(t-1)}}
$$

where the first term $\hat{\mu}_i(t) = (\sum_{c=1}^t \mathbb{I}(A_c = i) X_c) /
N_i(t)$ represents the estimation of $\mu_i$ at time $t$, and the second
explorative term $\sqrt{2 \log (t) / N_i(t)}$ denotes the confidence bound. UCB
satisfies \textit{sub-UCB} requirement as shown in \cite{auer2002finite}. UCB is
also an \textit{anytime} policy, which means it does not depend on the horizon
$T$.


\section{Related Work}
\label{sec:relate}

\textbf{Multi-armed bandits.} MAB \cite{slivkins_tutorial} is a simple yet
powerful framework for decision making under uncertainty. Let $r_{ti}$
represents reward on time $t$ at arm $i$, there are many categories of bandit
problems. Stochastic bandits \cite{gittins1979bandit, lai1985asymptotically,
	katehakis1987multi}, as the most classical one, assumes $\forall t, r_{ti}$ are
samples drawn from a stationary sub-gaussian distribution bound to bandit $i$.
Adversarial bandits \cite{auer1995gambling} assumes $\forall t, r_{ti}$ don't
have to belong to any stationary distribution and can be set by an adversary. It
is common to model $r_{ti}$ as a secret codebook set by an enemy who knows the
policy before playing. Contextual bandits \cite{langford2007epoch} introduces an
observable context variable and assumes $r_{ti}$ is drawn a distribution
parameterized by both bandit $i$ and context variable. There are many other
variants under the MAB framework, which we won't go into details. In this paper,
we focus on the stochastic bandits problem.


\textbf{UCB variants.} Upon being proposed, UCB \cite{auer2002finite} has
received strong research interests and developed into a large family of
policies. For example, KL-UCB \cite{garivier2011kl, cappe2013kullback} and
KL-UCB++ \cite{menard2017minimax} transform the UCB policy as a procedure that
calculates the best possible arm within a Kullback-Leibler divergence bound at
each time step. UCBV-Tune \cite{audibert2009exploration} incorporates variance
in place of unit variance assumption.

Particularly in the context of this paper, there have been several existing work
on redesigning the confidence bound. MOSS \cite{audibert2010regret} makes the
confidence bound depends on the number of plays for each bandit by replacing
$\log(t)$ with $\log(t / N_i(t))$, and policies similar to MOSS include OCUCB
\cite{lattimore2016regret} and UCB*
\cite{garivier2016explore}. UCB$\dagger$
\cite{lattimore2018refining} improves the previous ones significantly by
designing more advanced log function component.

Compared with these previous approaches, our method works differently by
extending the denominator term rather than the $\log$ function. It turns out to
be intuitive in foresight and deliver strong performance. Moreover, instead of
being non-parametric like most of the above methods, our policy has parameters
which are tunable, which indicates that the formulation of our method can be
extended into a family of policies.

% We show that it is easy to design a policy
% with better regret bound than UCB among this family.




\section{Method}


\subsection{Intuition}
\label{sec:intuition}

The idea here is when a bandit is pulled, instead of increasing the confidence
bound of other bandits uniformly, we shall increase more for
bandits who are similar to the current chosen bandit and vice versa.
On the one hand, it is reasonable in the sense of opportunity costs for not trying a
similar option. On the other hand, since the presence of mean estimation term,
this strategy will naturally lean towards and spend exploration budget on
similarly good bandits and save unnecessary trials from poor bandits.


To realize this idea, we start by looking at the confidence bound term $\sqrt{2
	\log (t) / N_i(t)}$ for $B_i$. Suppose there exists a measure function $d(i, j)$
ranges $[0, 1]$ that compares the distance between $B_i$ and $B_j$. Then we find
the idea can be implemented by replacing $N_i(t)$ as

\begin{equation}
	\begin{split}
		N_i(t) \Rightarrow  N_i(t) + \sum_{j \in [k] / i} d(i, j) N_j(t)
	\end{split}
	\label{eq:Ntilde}
\end{equation}

This modification can shrink confidence bounds of bandits which are
distant to others, while maintaining confidence bounds
of those close ones for further exploration.


Furthermore, this modification elegantly depicts the poles of exploration
and exploitation as

\begin{description}
	\item[Exploration] When $d(i, j) \equiv 0$, Eq. \ref{eq:Ntilde} will
	degrade to the vanilla UCB case, which is an "optimistic" policy and
	encourages exploration. We will revisit this topic in Sec. \ref{sec:under_exploration}.
	\item[Exploitation] When $d(i, j) \equiv 1$, Eq. \ref{eq:Ntilde} will degrade to greedy case because $N_i(t) = t$ and $\log (t) /
	t$ can rapidly converge to 0, which purely exploits.
\end{description}



\begin{wrapfigure}[12]{R}{0.57\textwidth}
	\centering
	\begin{minipage}{0.9\linewidth}
		\begin{algorithm}[H]
			% \SetAlgoLined
			\SetKwInOut{Input}{ input}
			\Input{distance measure $d_t$}
			\vspace*{-1em}
			\begin{equation*}
				\begin{split}
					A_t = \arg\max_{i\in[k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{ \widetilde{N}_i(t-1) }} \\
					\text{where } \widetilde{N}_i(t) = N_i(t) + \sum_{j \in [k] / i} d_t(i, j)  N_j(t)
				\end{split}
			\end{equation*}
			\caption{UCB-DT}
			\label{alg:ucbdt}
		\end{algorithm}
	\end{minipage}
\end{wrapfigure}


These two special cases correspond exactly to the simple and commonly recognized
truth: \textit{In the stochastic bandit problem, you shall explore just
enough to find the right bandit, then exploit that as long as you can.} 


While previous methods also encode similar principles, we can seamlessly model
the transition in our formulation. It indicates that if we could find a
transition from $d \equiv 0$ to $d \equiv 1$, like expanding $d$ from the origin
to a unit circle, then we can realize the above truth as well under the
framework in Eq.~\ref{eq:Ntilde}.


Therefore, we write $d$ as time dependent as $d_t$ and condense the above
findings in Alg. \ref{alg:ucbdt}. An example is provided to demonstrate our
ideas in Fig. \ref{fig:visual_example}. Specific instances of $d$ will be
introduced in Sec. \ref{sec:bdistance}.




\input{plots/intuition/plot.tex}


\subsection{Bandit Distances}

\label{sec:bdistance}

We design the following distance which composes UCB-DT($\mu$).

\begin{description}
	\item[UCB-DT($\mu$)] 
	\begin{equation}	
	d_t(i, j) =|\hat{\mu}_i(t) - \hat{\mu}_j(t)|^{1 / \floor{\gamma N_i(t)}}
	\label{eq:ucbdt}
	\end{equation}
\end{description}




First, it directly measures the distance between two bandits. Second, the more
times a bandit gets pulled, the closer its distances toward others approach to
1, which means the policy for this bandit transits deeper into exploitation from
exploration. And $\gamma$ is a speed parameter to control the transition rate.
It could be pointed that the UCB-DT($\mu$) will not work properly for bandits
whose $\mu_i \gg 1$ because the distance will saturate. But we argue that it is
common practice to use normalization to bypass this constraint. Thus, we keep
the above design for simplicity.

In the appendix \ref{apn:more_d}, we provide more designs for $d$ and analyze their
characteristics. In Fig.~\ref{fig:bandit_dist_vis}, we visualize the distance on
$N_i$ through different $\gamma$ and $|\hat{\mu}_i - \hat{\mu}_j|$.

\begin{figure}[H]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-2.pgf}
		}
	\end{minipage}
	\caption{Visualization of the Distance in Eq.~\ref{eq:ucbdt}. $\gamma$ is
	set to $0.02$ in the left figure, and $|\hat{\mu}_i - \hat{\mu}_j|$ is set to $0.2$ in
	the right figure. It is clear to see that the greater the
	difference between two bandits is, the
	faster that the distance is expanded from $0$ to $1$, speed of which can also be controlled
	by customizing $\gamma$.
	The curves are jagged because of the floor operation
	$\floor{\gamma N_i}$.}
	\label{fig:bandit_dist_vis}
\end{figure}




\subsection{Under Exploration Analysis}
\label{sec:under_exploration}

% Recall the \cite[Chapter~7]{lattimore2020bandit}, UCB is derived from
% Hoeffding's inequality on sum of subgaussian variables. With a slight abuse of
% notation, let $X_{1}, X_{2}, \ldots, X_{n}$ be independent and L1-subgaussian
% random variables with zero mean and $\hat{\mu}=\sum_{t=1}^{n} X_{t} / n$, then

% \vspace*{-1em}

% $$
% \mathbb{P}(\hat{\mu} \geq \varepsilon) \leq \exp \left(-n \varepsilon^{2} / 2\right)
% $$

% Replacing $\exp \left(-n \varepsilon^{2} / 2\right)$ with $\delta$ then we get

% \vspace*{-1em}

% $$
% \mathbb{P}\left(|\hat{\mu}| \geq \sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)} \right) \leq \delta
% $$

% If we use $1/t$ for $\delta$, we arrive to the formulation of UCB, where
% $\hat{\mu}$ denotes the shift between estimated mean and true mean, and we will
% write this shift for bandit $i$ as $\mshift{i}$. However, as we can see from
% Sec. \ref{sec:relate}, there are many research on redesigning the confidence
% bound term, and it is obvious that Alg. \ref{alg:ucbdt} actually under-explores
% than UCB. A natural question to ask is why the confidence bound needs to be
% modified if it is from the well-established concentration inequality?

Apparently, the Alg.~\ref{alg:ucbdt} under-explores than UCB to a large extent.
Thus, an immediate counter-argument to our idea can be
raised in the following.

\begin{center}
	\begin{fminipage}{0.8\textwidth}
		If the standard upper confidence bound is derived from the
		well-established concentration inequality, why under-exploration can be
		beneficial?
	\end{fminipage}
\end{center}

Previous work answer this question implicitly through regret bound analysis.
Through deriving a stricter upper bound on new methods than UCB, the rationality
of new methods are proven. We argue that many existing work
has been devoted to improving the $\log$ component because of the
analytical tractability of $\log$ function.

Despite that our method is concerned with the denominator instead of the $\log$
function and can be parameterized by $d$, we present a new perspective to answer
the above question which is also general enough to encompass different methods.

In the following, we suppose a scenario of two bandits where $\mu_1 > \mu_2$,
and we also assume $N_1 \ge N_2$. Since we only have two bandits, we can regard
$N_2(T)$ as the exploration budget spent till time $T$. We conduct our analysis by
hindsight\footnote{\quotes{By hindsight} means we look back at a policy's decisions from time $T$.} in the
context of standard UCB, but it shall be possible to extend to other methods.



\subsubsection{Exploration Full Point}

If we want to explore enough to ensure $P(A_T = 1) \ge 1 - \delta$, which means
we recognize the optimal bandit as the dominate choice. Then based on
Eq.~\ref{eq:ucb_dawn}, we need to have:

\begin{equation}
	P\left(\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)} \le \Delta_2 / 2\right) \le
	\delta
	\label{eq:full_inequality}
\end{equation}

where $\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)}$ is the
largest possible mean estimation deviation.
Since we have $\delta = 1/t$ in
UCB, we can solve for $N_2(T)$ when equality holds in
Eq.~\ref{eq:full_inequality}. 
To simplify notation, we skip $T$ in arguments:


\begin{equation}
	\begin{split}
		\sqrt{\frac{2}{N_2} \log \left(T\right)} & = \frac{\Delta_2}{2} \\
		N_{full} & = N_2 = \frac{8 \log(T)}{\Delta_2^2} 
	\end{split}
	\label{eq:exploration_full_point}
\end{equation}


The Eq.~\ref{eq:exploration_full_point} actually carries physical meaning, it
means if we explores for $N_{full}$ times, then the confidence bound will shrink
below to half of the suboptimality gap $\Delta_2$. Thus, we could safely choose
$B_1$, and any more exploration will be completely unnecessary.
To put in a succinct way of speaking, by exploring $N_{full}$
times according to the above equation, we fulfill the 
confidence bound of UCB.




Therefore, we write $N_2$ in Eq.~\ref{eq:exploration_full_point} as
\textit{Exploration Full Point} with $N_{full}$. Let $G_{full}$ denotes the
expected cumulated reward\footnote{For a simpler formulation, we use reward
	instead of regret for under exploration analysis.} at $N_{full}$:


\begin{equation}
	\begin{split}
		G_{full} = (T - N_{full}) \mu_1 + N_{full} \mu_2
	\end{split}
	\label{eq:gain_full}
\end{equation}


\subsubsection{Exploration Bargain Point} 


Instead of fulfilling the UCB confidence bound, what if we disobey it and stop
exploring before $N_{full}$? Clearly, we may lose reward by choosing $B_2$, but
meanwhile we save exploration budget. We can write a lower bound for expected
cumulated reward as $G(N_2)$:


\begin{equation}
	\begin{split}
		G(N_2) & \ge \underbrace{\left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right)}_{\text{Correctly choose $B_1$ as the best one}} + \underbrace{\left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta}_{\text{Mistakenly choose $B_2$ as the best one}} \\
		\text{where } \delta & = e^{- N_2 \Delta^2_2 / 8} \text{ is from Eq.~\ref{eq:exploration_full_point}}
	\end{split}
	\label{eq:gain_bargain}
\end{equation}


The key insight is that we can solve for $N_2$ by letting $G_{full}$ equal to
the right hand side of Eq. \ref{eq:gain_bargain}:

\begin{equation}
	\begin{split}
		N_{bargain}  =  & \underset{N_2}{\text{ solution}}  \bigg\{ G_{full} = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta \bigg\}
	\end{split}
	\label{eq:solve_bargain}
\end{equation}
 

We write the
solution as \textit{Exploration Bargain Point} with $N_{bargain}$ because we achieve
at least the same expected reward by only exploring to the point of
$N_{bargain}$. We will continue the
discussion of the solution form in appendix \ref{apn:ebp_more}.


\begin{figure}
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g2.pgf}
		}
	\end{minipage}
	\caption{Examples to demonstrate the relationship between expected cumulated
		rewards and exploration budget $N_2$. It elegantly explains why the
		standard confidence bound is over-optimistic and renders
		unnecessary explorations, and why many latest methods need to explore
		less to do more. }

%  It graphically explains why many latest methods need to
	% explore less to do more than the standard UCB.
	\label{fig:example_ebp}
\end{figure}

In Fig. \ref{fig:example_ebp}, we visualize the relationship among $N_{full}$,
$N_{bargain}$, and $G(N_2)$ by examples. It is fascinating to see that the best
trade-off locates between $N_{bargain}$ and $N_{full}$ because of the concavity
of subgaussian distribution, and rewards will decrease when you explore towards
the full point. This actually answers the above question and provides a
viewpoint to justify why many methods, including ours, need to explore less to
do more. Moreover, based on Eq. \ref{eq:exploration_full_point} and Fig.
\ref{fig:example_ebp}, $N_{bargain}$ bounds to be small when $\Delta_2$ is large,
which provides basis for our intuition of spending less exploration budget on
bandits far away from the optimal one and vice versa in Sec.
\ref{sec:intuition}.

\subsection{Regret Analysis}
\label{sec:analysis}

% Let $\mathcal{P}$ denotes the set of policies which UCB-DT can represent through
% parameterization of $d$. Our aim is to show that it is easy to find a \textit{sub-UCB} policy
% $\pi \in \mathcal{P}$.

In this section, we offer finite time regret bound analysis for UCB-DT. For the
sake of clear notation, we write $N_{i}(t)$ as $N_{i}(n)$ in the following.
Suppose $\mu_1 > \mu_2 > .. > \mu_k$, we can tell from Eq. \ref{eq:regret} that
the task of bounding $R_t$ can be translated as bounding
$\mathbb{E}\left[N_{i}(t)\right], i\in[k]/1$.


To derive the finite bound for $\mathbb{E}\left[N_{i}(t)\right]$, the common practice is
divide it into two cases when we choose suboptimal bandit over the
optimal bandit:

\begin{enumerate}[label=(\Alph*)]
	\item $\mu_1$ is under estimated, so the optimal bandit $B_1$ appears worse.
	\item $\mu_i, i\in[k]/1$ is over estimated, so the non-optimal bandit $B_i$ appears better.
\end{enumerate}



\begin{equation}
	\hspace*{-20pt}
	\begin{aligned}
		N_{i}(n) = & \sum_{t=1}^{n} \mathbb{I}\left\{A_{t}=i\right\}                                                                                                                                                                                                                                                                                          \\
		\leq       & \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\}}_{\text{(A)}}+ \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{i}(t)+\sqrt{\frac{2 \log t}{\widetilde{N}_i(t)}} \geq \mu_{1}-\varepsilon \text { and } A_{t}=i\right\}}_{\text{(B)}} \\
	\end{aligned}
\end{equation}

Given $\widetilde{N}_i(t) \ge N_i(t)$, we can relax (B) by replacing
$\widetilde{N}_i(t)$ with $N_i(t)$, which makes it identical to the case of UCB
and automatically arrive to $1 + \frac{2(\log t+\sqrt{\pi \log
	t}+1)}{\left(\Delta_{i}-\varepsilon\right)^{2}}$ according to
\cite{lattimore2020bandit}. At the same time, we have $\widetilde{N}_i(t) \le
t$, but we cannot apply a similar procedure to (A) because directly replacing
$\widetilde{N}_i(t)$ with $t$ will make (A) grow much faster and violate the
\textit{sub-UCB} condition.

%, which we show in appendix \ref{apn:need_for_explore_as}.

\begin{assumption}
	There exists time step $\tau$, which ensures the policy chooses $A_1$ often enough:
																																																																																																																																																																																																							
	$$
	\tau=\min \left\{t \leq T: \sup _{s \geq t}\left|\hat{\mu}_{1}(s)-\mu_{1}\right|<\varepsilon\right\}
	$$
																																																																																																																																																																																																							
	\label{assumption:enough}
\end{assumption}

If we can leverage assumption \ref{assumption:enough}, then a simple observation
is that:


\begin{equation}
	\begin{aligned}
		\sum_{t=1}^{T} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\} &   
		\le  \tau + \sum_{t=\tau+1}^T \mathbb{I}\{ \mu_1 - \hat{\mu}_1(t) \ge \varepsilon + \delta \}
	\end{aligned}
\end{equation}

It is straightforward to see that $P( \mu_1 - \hat{\mu}_1(t) \ge \varepsilon +
\delta \mid t > \tau) = 0$, where $\sqrt{2\log(t) / t}$ is replaced with $\delta
> 0$. Therefore, the (A) can be bounded within $\tau$. Furthermore, if we let
bandit distribution be gaussian, then by the concentration Lemma 1 in
\cite{lattimore2018refining}, $\mathbb{E}[\tau] \le 1+9 / \varepsilon^{2}$. Thus
the regret of UCB-DT is clearly upper bounded with \textit{sub-UCB} requirement.


Take UCB-DT($\mu$) as an example, we can reach the assumption
\ref{assumption:enough} as long as $\gamma$ to be small enough. In fact, UCB-DT
can represent a family of policies through parameterization of $d$, and the
regret bound here only describes the boundary behavior as it approaches the vanilla UCB.
According to Sec. \ref{sec:under_exploration} and appendix \ref{apn:ebp_more},
there exists a parameter space of $d$ which can be used to customize towards better
exploration-exploitation trade-off. Therefore, instead of diving into a detailed
regret expression of any specific form, we provide a general analysis without
explicitly including the degree of freedom.


\section{Numerical Experiments}

We compare UCB-DT to UCB \cite{auer2002finite}, UCB$\dagger$
\cite{lattimore2018refining}, UCBV-Tune \cite{audibert2009exploration}, KL-UCB
\cite{garivier2011kl, cappe2013kullback} and KL-UCB++ \cite{menard2017minimax}.
Among these methods, UCB, UCB$\dagger$ and UCBV-Tune are our main comparisons,
though UCB-DT can also be readily extended to support variance adaption.
The remaining two methods, KL-UCB and KL-UCB++,  which delivers excellent
performance, are \textit{non-anytime} policies. Because of these structural
differences, we do not regard them as our main comparisons, but we still keep
them as important references.




\begin{table}[h]
	\centering
	\begin{tabular}{lrrrrrr}
		\hline
		Experiment      & KL-UCB & KL-UCB++        & UCBV-Tune & UCB$\dagger$ & UCB     & UCB-DT($\mu$)  \\
		\hline
		B5 *            & 41.73  & \textbf{38.03}  & 98.6      & 129.01       & 251.28  & 70.95          \\
		B20 *           & 168.54 & \textbf{129.5}  & 415.23    & 410.5        & 939.99  & 383.82         \\
		B(0.02, 0.01) * & 28.34  & 22.39           & 64.99     & 131.99       & 249.17  & \textbf{21.6}  \\
		B(0.9, 0.88) *  & 38.44  & 33.78           & 49.6      & 73.9         & 119.91  & \textbf{19.19} \\
		N5 *            & 194.82 & 109.75          & 119.97    & 88.3         & 142.21  & \textbf{83.65} \\
		N20             & 539.91 & \textbf{410.25} & 840.26    & 560.47       & 1014.27 & 640.52         \\
		\hline
	\end{tabular}
	\vspace*{2pt}
	\caption{Regret of different policies in each environment.
		For each environment, we mark bold text for the best result and "*" if
		UCB-DT outperforms UCB, UCB$\dagger$ and UCBV-Tune.}
	\label{tab:regret}
\end{table}

For thorough experimentation, we design 6 environments as below

\begin{description}[leftmargin=!,labelwidth=\widthof{\bfseries B(0.02, 0.01)}]
	\item[B5] Bernoulli reward, 5 bandits with expected rewards 0.9, 0.8, 0.7, 0.2,
	0.5. This environment is modified from \cite{garivier2011kl} by adding more bandits.
	\item[B20] Bernoulli reward, 20 bandits with expected rewards 0.9, 0.85, 0.8, 0.8, 0.7,
	0.65, 0.6, 0.6, 0.55, 0.5,
	0.4, 0.4, 0.35, 0.3, 0.3,
	0.25, 0.2, 0.15, 0.1, 0.05, to test the
	case of many bandits.
	\item[B(0.02, 0.01)] Bernoulli reward, 3 bandits with expected rewards 0.05,
	0.02, 0.01, to test the case of low rewards. This environment is borrowed
	identically from \cite{garivier2011kl}.
	\item[B(0.9, 0.88)] Bernoulli reward, 2 bandits with expected rewards 0.9,
	0.88, to test the case of false commitment to sub-optimal arm.
	\item[N5] Gaussian reward, 5 bandits with unit variance and expected rewards
	1, 0.8, 0.5, 0.3, -0.2.
	\item[N20] Gaussian reward, 20 bandits with unit variance and expected rewards
	0, -0.03, -0.03, -0.07, -0.07, -0.07, -0.15, -0.15, -0.15, -0.5, -0.5, -0.5,
	-0.5, -0.5, -0.5, -0.5, -0.5, -0.5, -1, -1, to test the case of many bandits
	and low rewards and high variance. This environment is borrow identically
	from \cite{lattimore2018refining}.
\end{description}



We set $T$ to 20000 and run 2000 simulations for each method on every
environment. We do not specifically adjust the speed parameter, and we set
$\gamma$ to 0.02 in all experiments. For other methods, we use implementations
and default parameters from \cite{SMPyBandits}. We summarize cumulated regrets
in table \ref{tab:regret} and Fig. \ref{fig:exp}.


\begin{figure}[h]
	\centering
	\scalebox{0.33}{
		\input{plots/pgf_link/regrets.pgf}
	}
	\caption{Regret of different policies as a function of time (log scale) in each environment.}
	\label{fig:exp}
\end{figure}

From experiment results, we can see that UCB-DT is always better than UCB and
outperforms UCB$\dagger$, UCBV-Tune in 5 environments. We speculate the reason
of smaller improvement margin in N20 comes from the high variance of the 
environment, which makes the estimation of distance unstable. This behavior can
be alleviated with different distance designs as in appendix \ref{apn:more_d}.

% \section{Related Work}

\section{Conclusion}

By leveraging bandit distance, we create a policy called UCB-DT, which is
simple, extensible and performant. With analysis of our policy, we propose
the concept of \textit{Exploration Bargain Point} to provide a new perspective
on the confidence bound and exploration-exploitation trade-off.

Admittedly, this work bears its own limitations. We only study the
\textit{Exploration Bargain Point} in the context of two but not $K$ bandits.
The regret bound analysis is still not tight enough, and we lack a strict
formulation on the relationship between convergence behavior and possible
properties of $d$.

However, we believe these limitations could be regarded as future possibilities
in this direction, and it is also possibly promising to adopt the idea in this paper to
more general settings like adversarial bandit and reinforcement learning.



==> include.backup0920/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks [hidelinks]
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{algorithmic}
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{wrapfig}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage[boxruled]{algorithm2e}
\usepackage{enumitem}
\usepackage{float}

\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{caption}
\usepackage{subcaption}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand\tocite[1]{\textcolor{red}{[#1]}}
\newcommand\tosupple[1]{\textcolor{red}{[supplement #1]}}
\newcommand\mshift[1]{\hat{\mu}_{\Delta_{#1}}}

\newtheorem{assumption}{Assumption}
\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


%% This part goes in preamble
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


\newcommand{\quotes}[1]{``#1''}

==> include.backup0925/author.tex <==

\hypersetup{
	pdftitle={Tuning Confidence Bound for Stochastic Bandits with Bandit Distance},
	pdfsubject={statistics},
	pdfauthor={Xinyu Zhang},
	pdfkeywords={Multi-Armed Bandits, UCB, Confidence Bound},
	}

	
\title{Tuning Confidence Bound for Stochastic Bandits with Bandit Distance}


\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@eng.ucsd.edu}
	\And
	Srinjoy Das\\
	West Virginia University\\
	\texttt{srinjoy.das@mail.wvu.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@eng.ucsd.edu} 
}


==> include.backup0925/body.tex <==

\begin{abstract}
	We discover a novel modification upon the standard UCB method, which tunes
	confidence bound using bandit distance. Our formulation is simple to
	understand, straightforward for bound analysis, extensible, and naturally
	models the transition from exploration to exploitation. Our proposed
	distance measure can be customized to control the transition speed. We
	empirically demonstrate its strong performance over many latest methods.
	Along with the analysis of our method, we propose a new concept called
	\textit{Exploration Bargain Point} to intuitively explain why under
	exploration can be beneficial for upper confidence bound methods.
																																																																																																																																																																																																							
\end{abstract}


\section{Introduction}


Multi-armed bandit (MAB) problem \citep{slivkins_tutorial} can model a broad
range of applications, such as selecting the best website layout for users, or
choosing the most profitable stocks among many. Stochastic bandits is the
fundamental model of MAB, and one of the most influential and widely used
stochastic bandit policy is upper confidence bound method (UCB)
\citep{auer2002finite}. UCB works by maintaining a mean estimation and confidence
radius\footnote{We will refer confidence radius as confidence bound in the rest
of the paper.} for each bandit, and selecting the bandit with maximum sum of
mean and confidence bound at each step. The confidence bound can grow larger for
less-frequently used bandits which represents a higher degree of uncertainty to
serve the exploration purpose.


% However, UCB could waste many trials on non-optimal bandits by being optimistic
% indiscriminately. 

However, UCB by nature leads to unsatisfactory results  by being
over-optimistic on non-optimal bandits. In this work, we propose a simple
modification to the original UCB method which makes the confidence bound of one
bandit depends on its distance to others. Since the policy will select the
largest bandit more often, so the exploration will naturally lean towards the
neighbor of the largest bandit and save attempts from bad ones. An example is
provided in Fig. \ref{fig:intro}.


\begin{figure}[h]
	\vspace*{-8pt}
	\centering
	\scalebox{0.30}{
		\input{plots/pgf/intro_graph.pgf}
	}
	\vspace*{-8pt}
	\caption{Confidence bound comparison to UCB in a two-arm Bernoulli setting. By
	tunning confidence bound, the policy attempts fewer on the non-optimal one.}
	\label{fig:intro}
\end{figure}



By introducing bandit distance, we offer the opportunity of customization over policies
through different distances. Therefore, our formulation can represent a family of policies
which inherently model the transition from pro-exploration policy, such as UCB, to
pro-exploitation policy like greedy.


Moreover, many existing methods, including ours, redesign confidence bound to
under-explore than UCB. An interesting question can be asked: What is the drawback of using
the standard confidence bound if it is derived from the well-established concentration
inequality? 
Previous methods answer this implicitly by proving stricter 
regret bound. However, they are are neither straightforward nor intuitive
enough, while intuition undoubtedly can help us to gain deeper understanding and
improve a system. In this
paper, we present a novel concept named \textit{Exploration Bargain
Point} to answer this question directly and even graphically from a new
perspective. 



There are many existing work about the design of confidence bound, which we
will discuss in Sec. \ref{sec:relate}. While having connections to these
previous successive approaches, we make the following contributions in this paper.


\begin{itemize}
	\item We propose a new UCB-based policy, which tunes confidence bound by
	      bandit distance. We conduct analysis and numerical experiments to show our
	      formulation is simple, extensible, and performant.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
	\item We present a novel concept called \textit{Exploration Bargain Point},
	      which provides a new viewpoint of analysis on why exploration should
	      early stop in the context of upper confidence bound methods.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
\end{itemize}


\section{Preliminaries}



Let $k \in \mathbb{Z}^+$ be the number of bandits, $T$ denote the time horizon,
$\mu_i \in \mathbb{R}$ be the unknown mean for the distribution of bandit $i$,
$\mu_* = \max_i \mu_i$ be the mean of the optimal bandit, $B_i$ be the shorthand
for \quotes{bandit $i$} where $i\in[k]$. In each round $t \in [T] = \{1,2,...,T\}$, the policy
chooses a bandit $A_t \in [k]$ and receives an observation denoted by random
variable $X_t$.



We use $\Delta_i = \mu_* - \mu_i$ to represent the suboptimality gap for $i$th
bandit, and $N_i(t)$ to represent the number of times bandit $i$ gets chosen till $t$.
The regret over $T$ rounds is

\vspace*{-0.5em}

\begin{equation}
	\mathcal{R}_{T}=\sum_{i=1}^k \Delta_{i} \mathbb{E}\left[N_{i}(T)\right]
	\label{eq:regret}
\end{equation}

\vspace*{-0.5em}


which serves as the main metric for stochastic bandit policies. A policy is
called \textit{asymptotically optimal} if

\vspace*{-.5em}


$$
\lim _{T \rightarrow \infty} \frac{\mathcal{R}_{T}}{\log (T)}=\sum_{i: \Delta_{i}>0} \frac{2}{\Delta_{i}}
$$


% \vspace*{-.5em}



\citep{lai1985asymptotically,burnetas1997optimal} show that the above forms a
regret upper bound for all consistent policies. A policy is called
\textit{sub-UCB} \citep{lattimore2018refining}, which is a stricter requirement
than \textit{asymptotically optimality}, if there exists universal constants
$C_1, C_2 > 0$, the regret can be finitely bounded as

\vspace*{-0.5em}

$$
\mathcal{R}_{t} \leq C_{1} \sum_{i=1}^{k} \Delta_{i} + C_{2} \sum_{i: \Delta_{i}(\mu)>0} \frac{\log (n)}{\Delta_{i}}
$$


The UCB policy works by choosing bandit $A_t$ that


\vspace*{-.5em}


$$
A_t = \arg\max_{i \in [k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{N_i(t-1)}}
$$

where the first term $\hat{\mu}_i(t) = (\sum_{c=1}^t \mathbb{I}(A_c = i) X_c) /
N_i(t)$ represents the estimation of $\mu_i$ at time $t$, and the second
explorative term $\sqrt{2 \log (t) / N_i(t)}$ denotes the confidence bound. UCB
satisfies \textit{sub-UCB} requirement as shown in \citep{auer2002finite}. UCB is
also an \textit{anytime} policy, which means it does not depend on the horizon
$T$.


\section{Related Work}
\label{sec:relate}

\textbf{Multi-armed bandits.} MAB \citep{slivkins_tutorial} is a simple yet
powerful framework for decision making under uncertainty. Let $r_{ti}$
represents reward on time $t$ at arm $i$, there are many categories of bandit
problems. Stochastic bandits \citep{gittins1979bandit, lai1985asymptotically,
	katehakis1987multi}, as the most classical one, assumes $\forall t, r_{ti}$ are
samples drawn from a stationary sub-gaussian distribution bound to bandit $i$.
Adversarial bandits \citep{auer1995gambling} assumes $\forall t, r_{ti}$ don't
have to belong to any stationary distribution and can be set by an adversary. It
is common to model $r_{ti}$ as a secret codebook set by an enemy who knows the
policy before playing. Contextual bandits \citep{langford2007epoch} introduces an
observable context variable and assumes $r_{ti}$ is drawn a distribution
parameterized by both bandit $i$ and context variable. There are many other
variants under the MAB framework, which we won't go into details. In this paper,
we focus on the stochastic bandits problem.


\textbf{UCB variants.} Upon being proposed, UCB \citep{auer2002finite} has
received strong research interests and developed into a large family of
policies. For example, KL-UCB \citep{garivier2011kl, cappe2013kullback} and
KL-UCB++ \citep{menard2017minimax} transform the UCB policy as a procedure that
calculates the best possible arm within a Kullback-Leibler divergence bound at
each time step. UCBV-Tune \citep{audibert2009exploration} incorporates variance
in place of unit variance assumption.

Particularly in the context of this paper, there have been several existing work
on redesigning the confidence bound. MOSS \citep{audibert2010regret} makes the
confidence bound depends on the number of plays for each bandit by replacing
$\log(t)$ with $\log(t / N_i(t))$, and policies similar to MOSS include OCUCB
\citep{lattimore2016regret} and UCB*
\citep{garivier2016explore}. UCB$\dagger$
\citep{lattimore2018refining} improves the previous ones significantly by
designing more advanced log function component.

Compared with these previous approaches, our method works differently by
extending the denominator term rather than the $\log$ function. It turns out to
be intuitive in foresight and deliver strong performance. Moreover, instead of
being non-parametric like most of the above methods, our policy has parameters
which are tunable, which indicates that the formulation of our method can be
extended into a family of policies.

% We show that it is easy to design a policy
% with better regret bound than UCB among this family.




\section{Method}


\subsection{Intuition}
\label{sec:intuition}

The idea here is when a bandit is pulled, instead of increasing the confidence
bound of other bandits uniformly, we shall increase more for
bandits who are similar to the current chosen bandit and vice versa.
On the one hand, it is reasonable in the sense of opportunity costs for not trying a
similar option. On the other hand, since the presence of mean estimation term,
this strategy will naturally lean towards and spend exploration budget on
similarly good bandits and save unnecessary trials from poor bandits.


To realize this idea, we start by looking at the confidence bound term $\sqrt{2
	\log (t) / N_i(t)}$ for $B_i$. Suppose there exists a measure function $d(i, j)$
ranges $[0, 1]$ that compares the distance between $B_i$ and $B_j$. Then we find
the idea can be implemented by replacing $N_i(t)$ as

\begin{equation}
	\begin{split}
		N_i(t) \Rightarrow  N_i(t) + \sum_{j \in [k] / i} d(i, j) N_j(t)
	\end{split}
	\label{eq:Ntilde}
\end{equation}

This modification can shrink confidence bounds of bandits which are
distant to others, while maintaining confidence bounds
of those close ones for further exploration.


Furthermore, this modification elegantly depicts the poles of exploration
and exploitation as

\begin{description}
	\item[Exploration] When $d(i, j) \equiv 0$, Eq. \ref{eq:Ntilde} will
	degrade to the vanilla UCB case, which is an "optimistic" policy and
	encourages exploration. We will revisit this topic in Sec. \ref{sec:under_exploration}.
	\item[Exploitation] When $d(i, j) \equiv 1$, Eq. \ref{eq:Ntilde} will degrade to greedy case because $N_i(t) = t$ and $\log (t) /
	t$ can rapidly converge to 0, which purely exploits.
\end{description}



\begin{wrapfigure}[12]{R}{0.57\textwidth}
	\centering
	\begin{minipage}{0.9\linewidth}
		\begin{algorithm}[H]
			% \SetAlgoLined
			\SetKwInOut{Input}{ input}
			\Input{distance measure $d_t$}
			\vspace*{-1em}
			\begin{equation*}
				\begin{split}
					A_t = \arg\max_{i\in[k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{ \widetilde{N}_i(t-1) }} \\
					\text{where } \widetilde{N}_i(t) = N_i(t) + \sum_{j \in [k] / i} d_t(i, j)  N_j(t)
				\end{split}
			\end{equation*}
			\caption{UCB-DT}
			\label{alg:ucbdt}
		\end{algorithm}
	\end{minipage}
\end{wrapfigure}


These two special cases correspond exactly to the simple and commonly recognized
truth: \textit{In the stochastic bandit problem, you shall explore just
enough to find the right bandit, then exploit that as long as you can.} 


While previous methods also encode similar principles, we can seamlessly model
the transition in our formulation. It indicates that if we could find a
transition from $d \equiv 0$ to $d \equiv 1$, like expanding $d$ from the origin
to a unit circle, then we can realize the above truth as well under the
framework in Eq.~\ref{eq:Ntilde}.


Therefore, we write $d$ as time dependent as $d_t$ and condense the above
findings in Alg. \ref{alg:ucbdt}. An example is provided to demonstrate our
ideas in Fig. \ref{fig:visual_example}. Specific instances of $d$ will be
introduced in Sec. \ref{sec:bdistance}.




\input{plots/intuition/plot.tex}


\subsection{Bandit Distances}

\label{sec:bdistance}

We design the following distance which composes UCB-DT($\mu$).

\begin{description}
	\item[UCB-DT($\mu$)] 
	\begin{equation}	
	d_t(i, j) =|\hat{\mu}_i(t) - \hat{\mu}_j(t)|^{1 / \floor{\gamma N_i(t)}}
	\label{eq:ucbdt}
	\end{equation}
\end{description}




First, it directly measures the distance between two bandits. Second, the more
times a bandit gets pulled, the closer its distances toward others approach to
1, which means the policy for this bandit transits deeper into exploitation from
exploration. And $\gamma$ is a speed parameter to control the transition rate.
It could be pointed that the UCB-DT($\mu$) will not work properly for bandits
whose $\mu_i \gg 1$ because the distance will saturate. But we argue that it is
common practice to use normalization to bypass this constraint. Thus, we keep
the above design for simplicity.

In the appendix \ref{apn:more_d}, we provide more designs for $d$ and analyze their
characteristics. In Fig.~\ref{fig:bandit_dist_vis}, we visualize the distance on
$N_i$ through different $\gamma$ and $|\hat{\mu}_i - \hat{\mu}_j|$.

\begin{figure}[H]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-2.pgf}
		}
	\end{minipage}
	\caption{Visualization of the Distance in Eq.~\ref{eq:ucbdt}. $\gamma$ is
	set to $0.02$ in the left figure, and $|\hat{\mu}_i - \hat{\mu}_j|$ is set to $0.2$ in
	the right figure. It is clear to see that the greater the
	difference between two bandits is, the
	faster that the distance is expanded from $0$ to $1$, speed of which can also be controlled
	by customizing $\gamma$.
	The curves are jagged because of the floor operation
	$\floor{\gamma N_i}$.}
	\label{fig:bandit_dist_vis}
\end{figure}




\subsection{Under Exploration Analysis}
\label{sec:under_exploration}

% Recall the \citep[Chapter~7]{lattimore2020bandit}, UCB is derived from
% Hoeffding's inequality on sum of subgaussian variables. With a slight abuse of
% notation, let $X_{1}, X_{2}, \ldots, X_{n}$ be independent and L1-subgaussian
% random variables with zero mean and $\hat{\mu}=\sum_{t=1}^{n} X_{t} / n$, then

% \vspace*{-1em}

% $$
% \mathbb{P}(\hat{\mu} \geq \varepsilon) \leq \exp \left(-n \varepsilon^{2} / 2\right)
% $$

% Replacing $\exp \left(-n \varepsilon^{2} / 2\right)$ with $\delta$ then we get

% \vspace*{-1em}

% $$
% \mathbb{P}\left(|\hat{\mu}| \geq \sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)} \right) \leq \delta
% $$

% If we use $1/t$ for $\delta$, we arrive to the formulation of UCB, where
% $\hat{\mu}$ denotes the shift between estimated mean and true mean, and we will
% write this shift for bandit $i$ as $\mshift{i}$. However, as we can see from
% Sec. \ref{sec:relate}, there are many research on redesigning the confidence
% bound term, and it is obvious that Alg. \ref{alg:ucbdt} actually under-explores
% than UCB. A natural question to ask is why the confidence bound needs to be
% modified if it is from the well-established concentration inequality?

Apparently, the Alg.~\ref{alg:ucbdt} under-explores than UCB to a large extent.
Thus, an immediate counter-argument to our idea can be
raised in the following.

\begin{center}
	\begin{fminipage}{0.8\textwidth}
		If the standard upper confidence bound is derived from the
		well-established concentration inequality, why under-exploration can be
		beneficial?
	\end{fminipage}
\end{center}

Previous work answer this question implicitly through regret bound analysis.
Through deriving a stricter upper bound on new methods than UCB, the rationality
of new methods are proven. We argue that many existing work
has been devoted to improving the $\log$ component because of the
analytical tractability of $\log$ function.

Despite that our method is concerned with the denominator instead of the $\log$
function and can be parameterized by $d$, we present a new perspective to answer
the above question which is also general enough to encompass different methods.

In the following, we suppose a scenario of two bandits where $\mu_1 > \mu_2$,
and we also assume $N_1 \ge N_2$. Since we only have two bandits, we can regard
$N_2(T)$ as the exploration budget spent till time $T$. We conduct our analysis by
hindsight\footnote{\quotes{By hindsight} means we look back at a policy's decisions from time $T$.} in the
context of standard UCB, but it shall be possible to extend to other methods.



\subsubsection{Exploration Full Point}

If we want to explore enough to ensure $P(A_T = 1) \ge 1 - \delta$, which means
we recognize the optimal bandit as the dominate choice. Then based on
Eq.~\ref{eq:ucb_dawn}, we need to have:

\begin{equation}
	P\left(\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)} \le \Delta_2 / 2\right) \le
	\delta
	\label{eq:full_inequality}
\end{equation}

where $\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)}$ is the
largest possible mean estimation deviation.
Since we have $\delta = 1/t$ in
UCB, we can solve for $N_2(T)$ when equality holds in
Eq.~\ref{eq:full_inequality}. 
To simplify notation, we skip $T$ in arguments:


\begin{equation}
	\begin{split}
		\sqrt{\frac{2}{N_2} \log \left(T\right)} & = \frac{\Delta_2}{2} \\
		N_{full} & = N_2 = \frac{8 \log(T)}{\Delta_2^2} 
	\end{split}
	\label{eq:exploration_full_point}
\end{equation}


The Eq.~\ref{eq:exploration_full_point} actually carries physical meaning, it
means if we explores for $N_{full}$ times, then the confidence bound will shrink
below to half of the suboptimality gap $\Delta_2$. Thus, we could safely choose
$B_1$, and any more exploration will be completely unnecessary.
To put in a succinct way of speaking, by exploring $N_{full}$
times according to the above equation, we fulfill the 
confidence bound of UCB.




Therefore, we write $N_2$ in Eq.~\ref{eq:exploration_full_point} as
\textit{Exploration Full Point} with $N_{full}$. Let $G_{full}$ denotes the
expected cumulated reward\footnote{For a simpler formulation, we use reward
	instead of regret for under exploration analysis.} at $N_{full}$:


\begin{equation}
	\begin{split}
		G_{full} = (T - N_{full}) \mu_1 + N_{full} \mu_2
	\end{split}
	\label{eq:gain_full}
\end{equation}


\subsubsection{Exploration Bargain Point} 


Instead of fulfilling the UCB confidence bound, what if we disobey it and stop
exploring before $N_{full}$? Clearly, we may lose reward by choosing $B_2$, but
meanwhile we save exploration budget. We can write a lower bound for expected
cumulated reward as $G(N_2)$:


\begin{equation}
	\begin{split}
		G(N_2) & \ge \underbrace{\left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right)}_{\text{Correctly choose $B_1$ as the best one}} + \underbrace{\left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta}_{\text{Mistakenly choose $B_2$ as the best one}} \\
		\text{where } \delta & = e^{- N_2 \Delta^2_2 / 8} \text{ is from Eq.~\ref{eq:exploration_full_point}}
	\end{split}
	\label{eq:gain_bargain}
\end{equation}


The key insight is that we can solve for $N_2$ by letting $G_{full}$ equal to
the right hand side of Eq. \ref{eq:gain_bargain}:

\begin{equation}
	\begin{split}
		N_{bargain}  =  & \underset{N_2}{\text{ solution}}  \bigg\{ G_{full} = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta \bigg\}
	\end{split}
	\label{eq:solve_bargain}
\end{equation}
 

We write the
solution as \textit{Exploration Bargain Point} with $N_{bargain}$ because we achieve
at least the same expected reward by only exploring to the point of
$N_{bargain}$. We will continue the
discussion of the solution form in appendix \ref{apn:ebp_more}.


\begin{figure}
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g2.pgf}
		}
	\end{minipage}
	\caption{Examples to demonstrate the relationship between expected cumulated
		rewards and exploration budget $N_2$. It elegantly explains why the
		standard confidence bound is over-optimistic and renders
		unnecessary explorations, and why many latest methods need to explore
		less to do more. }

%  It graphically explains why many latest methods need to
	% explore less to do more than the standard UCB.
	\label{fig:example_ebp}
\end{figure}

In Fig. \ref{fig:example_ebp}, we visualize the relationship among $N_{full}$,
$N_{bargain}$, and $G(N_2)$ by examples. It is fascinating to see that the best
trade-off locates between $N_{bargain}$ and $N_{full}$ because of the concavity
of subgaussian distribution, and rewards will decrease when you explore towards
the full point. This actually answers the above question and provides a
viewpoint to justify why many methods, including ours, need to explore less to
do more. Moreover, based on Eq. \ref{eq:exploration_full_point} and Fig.
\ref{fig:example_ebp}, $N_{bargain}$ bounds to be small when $\Delta_2$ is large,
which provides basis for our intuition of spending less exploration budget on
bandits far away from the optimal one and vice versa in Sec.
\ref{sec:intuition}.

\subsection{Regret Analysis}
\label{sec:analysis}

% Let $\mathcal{P}$ denotes the set of policies which UCB-DT can represent through
% parameterization of $d$. Our aim is to show that it is easy to find a \textit{sub-UCB} policy
% $\pi \in \mathcal{P}$.

In this section, we offer finite time regret bound analysis for UCB-DT. For the
sake of clear notation, we write $N_{i}(t)$ as $N_{i}(n)$ in the following.
Suppose $\mu_1 > \mu_2 > .. > \mu_k$, we can tell from Eq. \ref{eq:regret} that
the task of bounding $R_t$ can be translated as bounding
$\mathbb{E}\left[N_{i}(t)\right], i\in[k]/1$.


To derive the finite bound for $\mathbb{E}\left[N_{i}(t)\right]$, the common practice is
divide it into two cases when we choose suboptimal bandit over the
optimal bandit:

\begin{enumerate}[label=(\Alph*)]
	\item $\mu_1$ is under estimated, so the optimal bandit $B_1$ appears worse.
	\item $\mu_i, i\in[k]/1$ is over estimated, so the non-optimal bandit $B_i$ appears better.
\end{enumerate}



\begin{equation}
	\hspace*{-20pt}
	\begin{aligned}
		N_{i}(n) = & \sum_{t=1}^{n} \mathbb{I}\left\{A_{t}=i\right\}                                                                                                                                                                                                                                                                                          \\
		\leq       & \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\}}_{\text{(A)}}+ \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{i}(t)+\sqrt{\frac{2 \log t}{\widetilde{N}_i(t)}} \geq \mu_{1}-\varepsilon \text { and } A_{t}=i\right\}}_{\text{(B)}} \\
	\end{aligned}
\end{equation}

Given $\widetilde{N}_i(t) \ge N_i(t)$, we can relax (B) by replacing
$\widetilde{N}_i(t)$ with $N_i(t)$, which makes it identical to the case of UCB
and automatically arrive to $1 + \frac{2(\log t+\sqrt{\pi \log
	t}+1)}{\left(\Delta_{i}-\varepsilon\right)^{2}}$ according to
\citep{lattimore2020bandit}. At the same time, we have $\widetilde{N}_i(t) \le
t$, but we cannot apply a similar procedure to (A) because directly replacing
$\widetilde{N}_i(t)$ with $t$ will make (A) grow much faster and violate the
\textit{sub-UCB} condition.

%, which we show in appendix \ref{apn:need_for_explore_as}.

\begin{assumption}
	There exists time step $\tau$, which ensures the policy chooses $A_1$ often enough:
																																																																																																																																																																																																							
	$$
	\tau=\min \left\{t \leq T: \sup _{s \geq t}\left|\hat{\mu}_{1}(s)-\mu_{1}\right|<\varepsilon\right\}
	$$
																																																																																																																																																																																																							
	\label{assumption:enough}
\end{assumption}

If we can leverage assumption \ref{assumption:enough}, then a simple observation
is that:


\begin{equation}
	\begin{aligned}
		\sum_{t=1}^{T} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\} &   
		\le  \tau + \sum_{t=\tau+1}^T \mathbb{I}\{ \mu_1 - \hat{\mu}_1(t) \ge \varepsilon + \delta \}
	\end{aligned}
\end{equation}

It is straightforward to see that $P( \mu_1 - \hat{\mu}_1(t) \ge \varepsilon +
\delta \mid t > \tau) = 0$, where $\sqrt{2\log(t) / t}$ is replaced with $\delta
> 0$. Therefore, the (A) can be bounded within $\tau$. Furthermore, if we let
bandit distribution be gaussian, then by the concentration Lemma 1 in
\citep{lattimore2018refining}, $\mathbb{E}[\tau] \le 1+9 / \varepsilon^{2}$. Thus
the regret of UCB-DT is clearly upper bounded with \textit{sub-UCB} requirement.


Take UCB-DT($\mu$) as an example, we can reach the assumption
\ref{assumption:enough} as long as $\gamma$ to be small enough. In fact, UCB-DT
can represent a family of policies through parameterization of $d$, and the
regret bound here only describes the boundary behavior as it approaches the vanilla UCB.
According to Sec. \ref{sec:under_exploration} and appendix \ref{apn:ebp_more},
there exists a parameter space of $d$ which can be used to customize towards better
exploration-exploitation trade-off. Therefore, instead of diving into a detailed
regret expression of any specific form, we provide a general analysis without
explicitly including the degree of freedom.


\section{Numerical Experiments}

We compare UCB-DT to UCB \citep{auer2002finite}, UCB$\dagger$
\citep{lattimore2018refining}, UCBV-Tune \citep{audibert2009exploration}, KL-UCB
\citep{garivier2011kl, cappe2013kullback} and KL-UCB++ \citep{menard2017minimax}.
Among these methods, UCB, UCB$\dagger$ and UCBV-Tune are our main comparisons,
though UCB-DT can also be readily extended to support variance adaption.
The remaining two methods, KL-UCB and KL-UCB++,  which delivers excellent
performance, are \textit{non-anytime} policies. Because of these structural
differences, we do not regard them as our main comparisons, but we still keep
them as important references.




\begin{table}[h]
	\centering
	\begin{tabular}{lrrrrrr}
		\hline
		Experiment      & KL-UCB & KL-UCB++        & UCBV-Tune & UCB$\dagger$ & UCB     & UCB-DT($\mu$)  \\
		\hline
		B5 *            & 41.73  & \textbf{38.03}  & 98.6      & 129.01       & 251.28  & 70.95          \\
		B20 *           & 168.54 & \textbf{129.5}  & 415.23    & 410.5        & 939.99  & 383.82         \\
		B(0.02, 0.01) * & 28.34  & 22.39           & 64.99     & 131.99       & 249.17  & \textbf{21.6}  \\
		B(0.9, 0.88) *  & 38.44  & 33.78           & 49.6      & 73.9         & 119.91  & \textbf{19.19} \\
		N5 *            & 194.82 & 109.75          & 119.97    & 88.3         & 142.21  & \textbf{83.65} \\
		N20             & 539.91 & \textbf{410.25} & 840.26    & 560.47       & 1014.27 & 640.52         \\
		\hline
	\end{tabular}
	\vspace*{2pt}
	\caption{Regret of different policies in each environment.
		For each environment, we mark bold text for the best result and "*" if
		UCB-DT outperforms UCB, UCB$\dagger$ and UCBV-Tune.}
	\label{tab:regret}
\end{table}

For thorough experimentation, we design 6 environments as below

\begin{description}[leftmargin=!,labelwidth=\widthof{\bfseries B(0.02, 0.01)}]
	\item[B5] Bernoulli reward, 5 bandits with expected rewards 0.9, 0.8, 0.7, 0.2,
	0.5. This environment is modified from \citep{garivier2011kl} by adding more bandits.
	\item[B20] Bernoulli reward, 20 bandits with expected rewards 0.9, 0.85, 0.8, 0.8, 0.7,
	0.65, 0.6, 0.6, 0.55, 0.5,
	0.4, 0.4, 0.35, 0.3, 0.3,
	0.25, 0.2, 0.15, 0.1, 0.05, to test the
	case of many bandits.
	\item[B(0.02, 0.01)] Bernoulli reward, 3 bandits with expected rewards 0.05,
	0.02, 0.01, to test the case of low rewards. This environment is borrowed
	identically from \citep{garivier2011kl}.
	\item[B(0.9, 0.88)] Bernoulli reward, 2 bandits with expected rewards 0.9,
	0.88, to test the case of false commitment to sub-optimal arm.
	\item[N5] Gaussian reward, 5 bandits with unit variance and expected rewards
	1, 0.8, 0.5, 0.3, -0.2.
	\item[N20] Gaussian reward, 20 bandits with unit variance and expected rewards
	0, -0.03, -0.03, -0.07, -0.07, -0.07, -0.15, -0.15, -0.15, -0.5, -0.5, -0.5,
	-0.5, -0.5, -0.5, -0.5, -0.5, -0.5, -1, -1, to test the case of many bandits
	and low rewards and high variance. This environment is borrow identically
	from \citep{lattimore2018refining}.
\end{description}



We set $T$ to 20000 and run 2000 simulations for each method on every
environment. We do not specifically adjust the speed parameter, and we set
$\gamma$ to 0.02 in all experiments. For other methods, we use implementations
and default parameters from \citep{SMPyBandits}. We summarize cumulated regrets
in table \ref{tab:regret} and Fig. \ref{fig:exp}.



From experiment results, we can see that UCB-DT is always better than UCB and
outperforms UCB$\dagger$, UCBV-Tune in 5 environments. We speculate the reason
of smaller improvement margin in N20 comes from the high variance of the 
environment, which makes the estimation of distance unstable. This behavior can
be alleviated with different distance designs as in appendix \ref{apn:more_d}.

% \section{Related Work}

\section{Conclusion}

By leveraging bandit distance, we create a policy called UCB-DT, which is
simple, extensible and performant. With analysis of our policy, we propose
the concept of \textit{Exploration Bargain Point} to provide a new perspective
on the confidence bound and exploration-exploitation trade-off.

Admittedly, this work bears its own limitations. We only study the
\textit{Exploration Bargain Point} in the context of two but not $K$ bandits.
The regret bound analysis is still not tight enough, and we lack a strict
formulation on the relationship between convergence behavior and possible
properties of $d$.

However, we believe these limitations could be regarded as future possibilities
in this direction, and it is also possibly promising to adopt the idea in this paper to
more general settings like adversarial bandit and reinforcement learning.



==> include.backup0925/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks [hidelinks]
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{algorithmic}
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{wrapfig}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage[boxruled]{algorithm2e}
\usepackage{enumitem}
\usepackage{float}

\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{caption}
\usepackage{subcaption}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand\tocite[1]{\textcolor{red}{[#1]}}
\newcommand\tosupple[1]{\textcolor{red}{[supplement #1]}}
\newcommand\mshift[1]{\hat{\mu}_{\Delta_{#1}}}

\newtheorem{assumption}{Assumption}
\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


%% This part goes in preamble
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


\newcommand{\quotes}[1]{``#1''}

==> include.backup1004/author.tex <==

\hypersetup{
	pdftitle={Tuning Confidence Bound for Stochastic Bandits with Bandit Distance},
	pdfsubject={statistics},
	pdfauthor={Xinyu Zhang},
	pdfkeywords={Multi-Armed Bandits, UCB, Confidence Bound},
	}

	
\title{Tuning Confidence Bound for Stochastic Bandits with Bandit Distance}


\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@eng.ucsd.edu}
	\And
	Srinjoy Das\\
	West Virginia University\\
	\texttt{srinjoy.das@mail.wvu.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@eng.ucsd.edu} 
}


==> include.backup1004/body.tex <==

\begin{abstract}
	We propose a novel modification of the standard upper confidence bound (UCB)
	method for the stochastic multi-armed bandit (MAB) problem which tunes the
	confidence bound of a given bandit based on its distance to others. Our UCB
	distance tuning (UCB-DT) formulation enables improved performance as
	measured by expected regret by preventing the MAB algorithm from focusing on
	non-optimal bandits which is a well-known deficiency of standard UCB.
	"Distance tuning" of the standard UCB is done using a proposed distance
	measure, which we call bandit distance, that is parameterizable and which
	therefore can be optimized to control the transition rate from exploration
	to exploitation based on problem requirements. We empirically demonstrate
	increased performance of UCB-DT versus many existing state-of-the-art
	methods which use the UCB formulation for the MAB problem. Our contribution
	also includes the development of a conceptual tool called the
	\textit{Exploration Bargain Point} which gives insights into the tradeoffs
	between exploration and exploitation. We argue that the exploration bargain
	point provides an intuitive perspective  that is useful for comparatively
	analyzing the performance of UCB-based methods.

	% We propose a novel modification of the standard UCB method for the
	% stochastic multi-armed bandit (MAB) problem which tunes the confidence bound
	% of a given bandit based on its distance to others. Our UCB-DT formulation
	% enables superior performance as measured by expected regret by preventing
	% the MAB algorithm from focusing on non-optimal bandits which is a well-known
	% deficiency of standard UCB. Our proposed distance measure which we call
	% bandit distance is parameterizable and can therefore be optimized to control
	% the transition rate from exploration to exploitation based on problem
	% requirements. We empirically demonstrate the strong performance of UCB-DT
	% versus many existing state-of-the-art methods which use the UCB formulation
	% for MAB. Our contribution also includes a concept called \textit{Exploration
	% Bargain Point} which provides insights into the tradeoffs between
	% exploration and exploitation thereby enabling an intuitive perspective
	% on analyzing the performance of UCB-based methods.
\end{abstract}


\section{Introduction}


Multi-armed bandit (MAB) \citep{slivkins_tutorial} can model a broad
range of applications, such as selecting the best website layout for users, or
choosing the most profitable stocks among many. Stochastic bandits is an
important setting in which MAB problems have been studied extensively. One of
the most influential and widely used stochastic bandit policy is the upper
confidence bound method (UCB) \citep{auer2002finite}. UCB works by maintaining a
mean estimation and confidence radius\footnote{We will refer confidence radius
as confidence bound in the rest of the paper.} for each bandit, and selects the
bandit whose sum of mean and confidence bound is the maximum among all bandits
at each step. The confidence bound can grow larger for less frequently used
bandits which represents a higher degree of uncertainty to serve the exploration
purpose.


% However, UCB could waste many trials on non-optimal bandits by being optimistic
% indiscriminately. 

However, the original UCB algorithm by its nature can lead to unsatisfactory
results by being over-optimistic on non-optimal bandits. In this work, we
propose UCB-DT (Upper Confidence Bound - Distance Tuning), a simple modification
to the original UCB method which makes the confidence bound of a given bandit
depend on its distance to others. Since the UCB-DT policy will select the
largest bandit more often, exploration will naturally lean towards the neighbors
of the largest bandit and prevent the algorithm from focusing on bandits that
are farther away. 

% An example
% is provided in Fig. \ref{fig:intro}.

% \begin{figure}[h]
% 	\vspace*{-8pt}
% 	\centering
% 	\scalebox{0.30}{
% 		\input{plots/pgf/intro_graph.pgf}
% 	}
% 	\vspace*{-8pt}
% 	\caption{Confidence bound comparison to UCB in a two-arm Bernoulli setting. By
% 	tunning confidence bound, the policy attempts fewer on the non-optimal one.}
% 	\label{fig:intro}
% \end{figure}



By introducing bandit distance, we offer the opportunity of customization over policies
through different distances. Therefore, our formulation can represent a family of policies
which inherently provide the flexibility of both pro-exploration policies, such as UCB, and
pro-exploitation policies like $\epsilon$-greedy.


Moreover, unlike previous methods which focus on the $\log$ function in 
confidence bound because of its analytical tractability, our
method works differently by extending the denominator term. To circumvent the
analytical difficulties, we propose a concept named \textit{Exploration Bargain
Point} to provide a novel perspective on analyzing performance of UCB-based
methods. With our new analysis tool, we intuitively and even graphically
show that our method can always perform better than standard UCB.






% Moreover, many existing methods, including ours, redesign confidence bound to
% under-explore than UCB. An interesting question can be asked: What is the
% drawback of using the standard confidence bound if it is derived from the
% well-established concentration inequality? Previous methods answer this
% implicitly by proving stricter regret bound. However, they are are neither
% straightforward nor intuitive enough, while intuition undoubtedly can help us to
% gain deeper understanding and improve a system. In this paper, we present a
% novel concept named \textit{Exploration Bargain Point} to answer this question
% directly and even graphically from a new perspective. 



There are many existing work about the design of confidence bound, which we
will discuss in Sec. \ref{sec:relate}. While having connections to these
previous successive approaches, we make the following contributions in this paper.


\begin{itemize}
	\item We propose a new UCB-based policy, which tunes confidence bound by
	      bandit distance. We conduct analysis and numerical experiments to show our
	      formulation is simple, extensible, and performant.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
	\item We present a concept called \textit{Exploration Bargain Point},
	      which provides a novel viewpoint on analyzing performance of upper
	      confidence bound methods.

		%   in the context of 
		%   why exploration should
	    %   early stop in the context of upper confidence bound methods.
	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      	      
\end{itemize}


\section{Preliminaries}



Let $k \in \mathbb{Z}^+$ be the number of bandits, $T$ denote the time horizon,
$\mu_i \in \mathbb{R}$ be the unknown mean for the subgaussian distribution of bandit $i$,
$\mu_* = \max_i \mu_i$ be the mean of the optimal bandit, $B_i$ be the shorthand
for \quotes{$i$th bandit} where $i\in[k]$. In each round $t \in [T] = \{1,2,...,T\}$, the policy
chooses a bandit $A_t \in [k]$ and receives an observation denoted by random
variable $X_t$.



We use $\Delta_i = \mu_* - \mu_i$ to represent the suboptimality gap for $B_i$, and $N_i(t)$ to represent the number of times bandit $i$ gets chosen till $t$.
The regret over $T$ rounds is

\vspace*{-1em}

\begin{equation}
	\mathcal{R}_{T}=\sum_{i=1}^k \Delta_{i} \mathbb{E}\left[N_{i}(T)\right]
	\label{eq:regret}
\end{equation}

\vspace*{-0.5em}


which serves as the main metric for stochastic bandit policies. A policy is
called \textit{asymptotically optimal} if

\vspace*{-1em}


\begin{equation}
\lim _{T \rightarrow \infty} \frac{\mathcal{R}_{T}}{\log (T)}=\sum_{i: \Delta_{i}>0} \frac{2}{\Delta_{i}}
\label{eq:regret_bound}
\end{equation}


% \vspace*{-.5em}



\citep{lai1985asymptotically,burnetas1997optimal} show that the above forms a
regret upper bound for all consistent policies. A policy is called
\textit{sub-UCB} \citep{lattimore2018refining}, which is a stricter requirement
than \textit{asymptotically optimality}, if there exists universal constants
$C_1, C_2 > 0$, the regret can be finitely bounded as

\vspace*{-1em}

\begin{equation}
\mathcal{R}_{t} \leq C_{1} \sum_{i=1}^{k} \Delta_{i} + C_{2} \sum_{i: \Delta_{i}(\mu)>0} \frac{\log (n)}{\Delta_{i}}
\label{eq:regret_bound_finite}
\end{equation}


The UCB policy works by choosing bandit $A_t$ that


\vspace*{-1em}

\begin{equation}
A_t = \arg\max_{i \in [k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{N_i(t-1)}}
\label{eq:ucb}
\end{equation}

\vspace*{-.5em}

where the first term $\hat{\mu}_i(t) = (\sum_{c=1}^t \mathbb{I}(A_c = i) X_c) /
N_i(t)$ represents the estimation of $\mu_i$ at time $t$, and the second
explorative term $\sqrt{2 \log (t) / N_i(t)}$ denotes the confidence bound. UCB
satisfies \textit{sub-UCB} requirement as shown in \citep{auer2002finite}. UCB is
also an \textit{anytime} policy, which does not depend on the horizon
$T$.


\section{Related Work}
\label{sec:relate}

\textbf{Multi-armed bandits.} MAB \citep{slivkins_tutorial} is a simple yet
powerful framework for decision making under uncertainty. Let $r_{ti}$
represents reward on time $t$ at arm $i$, there are many categories of bandit
problems. Stochastic bandits \citep{gittins1979bandit, lai1985asymptotically,
katehakis1987multi}, as the most classical one, assumes $\forall t, r_{ti}$ are
samples drawn from a stationary sub-gaussian distribution bound to bandit $i$.
Adversarial bandits \citep{auer1995gambling} assumes $\forall t, r_{ti}$ don't
have to belong to any stationary distribution and can be set by an adversary. It
is common to model $r_{ti}$ as a secret codebook set by an enemy who knows the
policy before playing. Contextual bandits \citep{langford2007epoch} introduces
an observable context variable and assumes $r_{ti}$ is drawn a distribution
parameterized by both bandit $i$ and context variable. There are many other
variants under the MAB framework, whose details are beyond the scope of this
paper. In this paper, we focus on the stochastic bandits problem.


\textbf{UCB variants.} Since being first proposed, UCB \citep{auer2002finite} has
received strong research interest and several variants of the original UCB
policy have been proposed. For example, KL-UCB \citep{garivier2011kl, cappe2013kullback} and
KL-UCB++ \citep{menard2017minimax} transform the UCB policy as a procedure that
calculates the best possible arm within a Kullback-Leibler divergence bound at
each time step. UCBV-Tune \citep{audibert2009exploration} incorporates variance
in place of unit variance assumption.

Particularly in the context of this paper, there have been several existing work
on redesigning the confidence bound. MOSS \citep{audibert2010regret} makes the
confidence bound depends on the number of plays for each bandit by replacing
$\log(t)$ with $\log(t / N_i(t))$, and policies similar to MOSS include OCUCB
\citep{lattimore2016regret} and UCB*
\citep{garivier2016explore}. UCB$\dagger$
\citep{lattimore2018refining} improves the previous ones significantly by
designing more advanced log function component.

Compared with these previous approaches, our method works differently by
extending the denominator term rather than the $\log$ function. It turns out to
be intuitive in foresight and deliver strong performance. Moreover, instead of
being non-parametric like most of the above methods, our policy has parameters
which are tunable, which indicates that the formulation of our method can be
extended into a family of policies.

% We show that it is easy to design a policy
% with better regret bound than UCB among this family.




\section{Method}


\subsection{Intuition}
\label{sec:intuition}

The idea is when a bandit is selected, instead of increasing the confidence
bounds of all other bandits uniformly, we increase them more for bandits which
are similar to the current chosen bandit and vice versa. The intuition is that a
similar bandit has a higher chance to be equally good as the current chosen
one. Since the presence of mean estimation term, this strategy will
naturally lean towards the optimal bandit and spend exploration budget on
similarly good bandits and save unnecessary trials from poor bandits.


To realize this idea, we start by looking at the confidence bound term $\sqrt{2
	\log (t) / N_i(t)}$ for $B_i$ in Eq.~\ref{eq:ucb}. Suppose there exists a
	distance measure $d(i, j)$
ranges between $[0, 1]$ that compares the distance between $B_i$ and $B_j$. Then we find
the above idea can be implemented by replacing $N_i(t)$ as

\begin{equation}
	\begin{split}
		N_i(t) \Rightarrow  N_i(t) + \sum_{j \in [k] / i} d(i, j) N_j(t)
	\end{split}
	\label{eq:Ntilde}
\end{equation}

This modification can shrink the confidence bounds of bandits which are
distant from others, while maintaining the confidence bounds
of those ones that are closer for further exploration.
Furthermore, this modification elegantly depicts the poles of exploration
and exploitation as below:

\begin{description}
	\item[Exploration] When $d(i, j) \equiv 0$, Eq. \ref{eq:Ntilde} will
	degrade to the vanilla UCB case, which is an "optimistic" policy and
	encourages exploration. %We will revisit this topic in Sec. \ref{sec:under_exploration}.
	\item[Exploitation] When $d(i, j) \equiv 1$, Eq. \ref{eq:Ntilde} will degrade to greedy case because $N_i(t) = t$ and $\log (t) /
	t$ can rapidly converge to 0, which purely exploits.
\end{description}



\begin{wrapfigure}[12]{R}{0.57\textwidth}
	\centering
	\begin{minipage}{0.9\linewidth}
		\begin{algorithm}[H]
			% \SetAlgoLined
			\SetKwInOut{Input}{ input}
			\Input{distance measure $d_t$}
			\vspace*{-1em}
			\begin{equation*}
				\begin{split}
					A_t = \arg\max_{i\in[k]} \hat{\mu}_i(t-1) + \sqrt{\frac{2 \log (t-1)}{ \widetilde{N}_i(t-1) }} \\
					\text{where } \widetilde{N}_i(t) = N_i(t) + \sum_{j \in [k] / i} d_t(i, j)  N_j(t)
				\end{split}
			\end{equation*}
			\caption{UCB distance tuning (UCB-DT)}
			\label{alg:ucbdt}
		\end{algorithm}
	\end{minipage}
\end{wrapfigure}


These two special cases correspond exactly to the simple and commonly recognized
truth: \textit{In the stochastic bandit problem, you shall explore just
enough to find the right bandit, then exploit that as long as you can.} 


% While previous methods also encode similar principles, we can seamlessly model
% the transition in our formulation. 

In our formulation, we can model this transition from exploration to
exploitation by customizing $d$. It indicates that if we could find a transition
from $d \equiv 0$ to $d \equiv 1$, like expanding $d$ from the origin to a unit
circle, then we can realize the above truth as well under the framework in
Eq.~\ref{eq:Ntilde}.


Therefore, we write $d$ as time dependent as $d_t$ and condense the above
findings in Alg. \ref{alg:ucbdt}. An example is provided to demonstrate our
ideas in Fig. \ref{fig:visual_example}. Specific instances of $d$ will be
introduced in Sec. \ref{sec:bdistance}.




\input{plots/intuition/plot.tex}


\subsection{Bandit Distance}

\label{sec:bdistance}

We design the following distance which composes UCB-DT($\mu$).

\begin{description}
	\item[UCB-DT($\mu$)] 
	\begin{equation}	
	d_t(i, j) =|\hat{\mu}_i(t) - \hat{\mu}_j(t)|^{1 / \floor{\gamma N_i(t)}}
	\label{eq:ucbdt}
	\end{equation}
\end{description}




First, it directly measures the distance between two bandits. Second, the more
times a bandit gets pulled, the closer its distances from all other bandits will
approach the maximum value of 1, which means that the policy for this bandit
transitions deeper into exploitation from exploration. And $\gamma$ is a speed
parameter to control the transition rate. It could be pointed that the
UCB-DT($\mu$) will not work properly for bandits whose $\mu_i \gg 1$ because the
distance will saturate. But we argue that it is common practice to use
normalization to bypass this constraint. Thus, we keep the above design for
simplicity.

In Appendix \ref{apn:more_d}, we provide more designs for $d$ and analyze their
characteristics. In Fig.~\ref{fig:bandit_dist_vis}, we visualize the distance on
$N_i$ through different $\gamma$ and $|\hat{\mu}_i - \hat{\mu}_j|$.

\begin{figure}[H]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/bandit-distance-2.pgf}
		}
	\end{minipage}
	\caption{Visualization of the Distance in Eq.~\ref{eq:ucbdt}. $\gamma$ is
	set to $0.02$ in the left figure, and $|\hat{\mu}_i - \hat{\mu}_j|$ is set to $0.2$ in
	the right figure. It can be clearly seen that the greater the
	difference between two bandits is, the
	faster that the distance is expanded from $0$ to $1$, speed of which can also be controlled
	by customizing $\gamma$.
	The curves are jagged because of the floor operation
	$\floor{\gamma N_i}$.}
	\label{fig:bandit_dist_vis}
\end{figure}




\subsection{Under Exploration Analysis}
\label{sec:under_exploration}

% 1. restructure 4.3
% 2. write a proof to show N2_bargain <= Nfull. then our algorithm can gives better than UCB
% 3. practical way to choose gamma

The Alg.~\ref{alg:ucbdt} under-explores than UCB to a large extent. In this
section, we conduct an analysis based on a novel concept called
\textit{Exploration Bargain Point} to show our method can always give better
performance than UCB. Based on our analysis tool, we provide practical
advice on how to set the $\gamma$ parameter. 


Previous work prove their advantage over UCB through regret bound analysis. We
argue that many existing work have been devoted to improving the $\log$ function 
because of its analytical tractability. 
Despite that our method is concerned with the denominator instead of the $\log$
function and can even be parameterized by $d$, our new analysis tool is general
enough to encompass our method.  



In the following, we suppose a scenario of two bandits where $\mu_1 > \mu_2$,
and we also assume $N_1 \ge N_2$. Since we only have two bandits, we can regard
$N_2(T)$ as the exploration budget spent till time $T$, and $T = N_1 + N_2$. We conduct our analysis by
hindsight\footnote{\quotes{By hindsight} means we look back at a policy's decisions from time $T$.} in the
context of standard UCB. %, but it shall be possible to extend to other methods.



\subsubsection{Exploration Full Point}

If we want to explore enough to ensure $P(A_T = 1) \ge 1 - \delta$, which means
we recognize the optimal bandit as the dominate choice. Then based on
Eq.~\ref{eq:ucb_dawn}, we need to have:

\begin{equation}
	P\left(\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)} \le \Delta_2 / 2\right) \le
	\delta
	\label{eq:full_inequality}
\end{equation}

where $\sqrt{\frac{2}{n} \log \left(\frac{1}{\delta}\right)}$ is the
largest possible deviation of mean estimation.
Since we have $\delta = 1/t$ in
UCB, we can solve for $N_2(T)$ when equality holds in
Eq.~\ref{eq:full_inequality}. 
To simplify notation, we skip $T$ in arguments:



\begin{equation}
	\begin{split}
		\sqrt{\frac{2}{N_2} \log \left(T\right)} & = \frac{\Delta_2}{2} \\
		N_{full} & = N_2 = \frac{8 \log(T)}{\Delta_2^2} 
	\end{split}
	\label{eq:exploration_full_point}
\end{equation}


The Eq.~\ref{eq:exploration_full_point} carries physical meaning, it
means if we explores for $N_{full}$ times, then the confidence bound will shrink
below to half of the suboptimality gap $\Delta_2$. Thus, we could safely choose
$B_1$, and any more exploration will be completely unnecessary.
To put in a succinct way of speaking, by exploring $N_{full}$
times according to the above equation, we fulfill the 
confidence bound of UCB.



Therefore, we write $N_2$ in Eq.~\ref{eq:exploration_full_point} as
\textit{Exploration Full Point} with $N_{full}$. Let $G_{full}$ denotes the
expected cumulative reward\footnote{For a simpler formulation, we use reward
	instead of regret for under exploration analysis.} at $N_{full}$:

\vspace{-1em}


\begin{equation}
	\begin{split}
		G_{full} = (T - N_{full}) \mu_1 + N_{full} \mu_2
	\end{split}
	\label{eq:gain_full}
\end{equation}


\subsubsection{Exploration Bargain Point} 
\label{sec:bargain_point}

The key question is could we stop exploring before $N_{full}$ and achieve better
performance? The trade-off is we could have a smaller $N_2$ by exploring less,
but the probability of recognizing the non-optimal bandit as the dominate choice
$P(A_T = 2) = \delta$ will grow larger and become non-negligible. Therefore,
with a slight abuse of notation, we can write a lower bound for expected
cumulative reward as $G(N_2)$:


\vspace{-1em}
\begin{equation}
	\begin{split}
		G(N_2) & \ge \underbrace{\left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right)}_{\text{Correctly choose $B_1$ as the best one}} 
		 \overbrace{\left(1 - \delta \right)}^{\scaleto{\inf P(A_T=1)}{0.6em}} + \underbrace{\left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right)}_{\text{Mistakenly choose $B_2$ as the best one}} \overbrace{\delta}^{{\scaleto{\sup P(A_T=2)}{0.6em}}} \\
		\text{where } \delta & = e^{- N_2 \Delta^2_2 / 8} \text{ is from Eq.~\ref{eq:exploration_full_point}}
	\end{split}
	\label{eq:gain_bargain}
\end{equation}

% Next, we can write the condition of better performance as 
Next, to ensure we can achieve better or at least the same performance as $N_{full}$, we write

\vspace{-1em}

\begin{equation}
	\begin{split}
		G(N_2) & \ge G_{full} \\ 
		% G_{full} & = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right)
		% \left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta
		% N_{bargain}  =  & \underset{N_2}{\text{ solution}}  \bigg\{ G_{full} = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta \bigg\}
	\end{split}
	\label{eq:gN2_ge_gfull}
\end{equation}
 
Then, to find out the boundary condition where the same performance are
achieved, we can let $G_{full}$ in Eq.~\ref{eq:gain_full} to equal the right
hand side of the Eq.~\ref{eq:gain_bargain}.

\vspace{-1em}

\begin{equation}
	\begin{split}
		G_{full} & = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right)
		\left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta
		% N_{bargain}  =  & \underset{N_2}{\text{ solution}}  \bigg\{ G_{full} = \left( \left(T - N_2 \right) \mu_1 + N_2 \mu_2 \right) \left(1 - \delta \right) + \left( \left(T - N_2 \right) \mu_2 + N_2 \mu_1 \right) \delta \bigg\}
	\end{split}
	\label{eq:gfull_eq_right}
\end{equation}

We write the
solution of Eq.~\ref{eq:gfull_eq_right} as \textit{Exploration Bargain Point}
with $N_{bargain} = \underset{N_2}{\text{ solution}}  \{ \text{Equation~\ref{eq:gfull_eq_right}} \}$ because we achieve
at least the same expected reward by only exploring to the point of
$N_{bargain}$. We continue the
 discussion of the solution form in Appendix \ref{apn:ebp_more}.

% \vspace{-1.5em}

% \begin{equation}
% 	\begin{split}
% 		N_{bargain}  =  & \underset{N_2}{\text{ solution}}  \bigg\{ \text{Equation~\ref{eq:gfull_eq_right}} \bigg\}
% 	\end{split}
% 	\label{eq:solve_bargain}
% \end{equation}


\begin{figure}
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g1.pgf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\input{plots/pgf_link/ebp/g2.pgf}
		}
	\end{minipage}
	\caption{Examples to demonstrate the relationship between expected cumulative
		reward $G(N_2)$ and exploration budget $N_2$}

	\label{fig:example_ebp}
\end{figure}


\textbf{Determine $\mathbf{\gamma}$ with $\mathbf{N_{bargain}}$.} In Fig.
\ref{fig:example_ebp}, we visualize the relationship among $N_{full}$,
$N_{bargain}$, and $G(N_2)$ by examples. It is fascinating to see that the
optimal exploration point locates between $N_{bargain}$ and $N_{full}$ because
of the concavity of subgaussian distribution. Therefore, our method can always
perform better than UCB as long as the $\gamma$ is set to $1 / N_{bargain}$ in
Eq.~\ref{eq:ucbdt}. It ensures that after exploring enough by pass $N_{bargain}$
(\textcolor{DarkRed}{red} dot), distance in Eq.~\ref{eq:ucbdt} will become
larger than 0, which makes the confidence bounds of all bandits in
Alg.~\ref{alg:ucbdt} smaller than that of UCB. By having smaller confidence
bounds, our policy will under-explore than UCB and stop before the $N_{full}$
(\textcolor{DarkGreen}{green} dot). Thus, the final $N_2$ will lie between
$N_{bargain}$ and $N_{full}$, where $G(N_2) > G_{full}$. Moreover, as shown by
Eq.~\ref{eq:transend}, $N_{bargain}$ only depends on suboptimality gap
$\Delta_2$ and time horizon $T$, and does not rely on the actual values of
$\mu_i$. We argue that domain knowledge could be used to estimate the difference
between optimal bandit and other ones in practice. In Sec.~\ref{sec:exp}, we set
$\gamma$ to be 0.02 in all experiments, which is equivalent to assume
$N_{bargain}$ to be 50.

\textbf{Existence of $\mathbf{N_{bargain}}$.} $N_{bargain}$ always exists as
long as $\mu_1 > \mu_2$, which can be proven by contradiction. Because of the
concavity of subgaussian distribution, the only possible case that $N_{bargain}$
does not exist is $N_{bargain} = N_{full}$, where the $G_{full}$
(\textcolor{YellowOrange}{orange} curve) becomes the tangent line of $G(N_2)$
(\textcolor{NavyBlue}{blue} curve). From Eq.~\ref{eq:gfull_eq_right}, we get

\vspace{-0.5em}
\small
\begin{equation}
	\begin{split}
		\left( \left(T - N_{full} \right) \mu_1 + N_{full} \mu_2 \right) = \left( \left(T - N_{full} \right) \mu_1 + N_{full} \mu_2 \right)
		\left(1 - \delta \right) + \left( \left(T - N_{full} \right) \mu_2 + N_{full} \mu_1 \right) \delta& 
	\end{split}
	\label{eq:existance_bargain}
\end{equation}
\normalsize
\vspace{-1em}

It follows directly that $\delta = 0$. Since $\delta = e^{- N_2 \Delta^2_2 / 8}$
from Eq.~\ref{eq:gain_bargain}, we get $N_2 = \inf$. Then, from
Eq.~\ref{eq:exploration_full_point}, $N_2 = \inf \rightarrow \Delta_2 = 0$.
However, we assume $\Delta_2 = \mu_1 - \mu_2 > 0$. So $N_{bargain}$ must always
exist. 



\textbf{Implications.} Exploration bargain point describes exactly the
over-exploring nature of UCB. We could use $N_{bargain}$ as an anchor to
optimize the UCB method:

\begin{itemize}
	\item It allows UCB practitioners to early stop and prevent
	over-exploration. We summarize this policy as UCB-then-Commit in
	Appendix~\ref{apn:more_d}. In Table~\ref{tab:more_dist}, we see that UCB-then-Commit
	outperforms UCB in most environments but is never as good as UCB-DT($\mu$).

	\item Leveraging $N_{bargain}$, UCB-DT($\mu$) knows when to cross into the
	optimal territory to get better reward. 
\end{itemize}

This insight is not available to the traditional regret bound analysis. We
believe our analysis tool provides a novel and more intuitive perspective on
analyzing UCB-based methods.

% In fact, both exploration full and bargain points
% describe exactly the \textit{worst case performance} of UCB and our method,
% which is also the core concept for traditional regret bound analysis. 


% traditional regret bound analysis. 
% We believe our analysis tool provides a novel and more intuitive perspective on analyzing
% UCB-based methods.




\subsection{Regret Analysis}
\label{sec:analysis}

% Let $\mathcal{P}$ denotes the set of policies which UCB-DT can represent through
% parameterization of $d$. Our aim is to show that it is easy to find a \textit{sub-UCB} policy
% $\pi \in \mathcal{P}$.

In addition to our analysis in Sec.~\ref{sec:under_exploration}, we offer a
finite time regret bound analysis for UCB-DT following standard practice. For
the sake of clear notation, we write $N_{i}(t)$ as $N_{i}(n)$. Suppose $\mu_1 >
\mu_2 > .. > \mu_k$, we can tell from Eq. \ref{eq:regret} that the task of
bounding $R_t$ can be translated as bounding $\mathbb{E}\left[N_{i}(t)\right],
i\in[k]/1$. The idea is divide it into two cases when we choose suboptimal
bandit over the optimal bandit:


% To derive the finite bound for $\mathbb{E}\left[N_{i}(t)\right]$, the idea is
% divide it into two cases when we choose suboptimal bandit over the
% optimal bandit:

\begin{enumerate}[label=(\Alph*)]
	\item $\mu_1$ is under estimated, so the optimal bandit $B_1$ appears worse.
	\item $\mu_i, i\in[k]/1$ is over estimated, so the non-optimal bandit $B_i$ appears better.
\end{enumerate}


\vspace{-1em}
\small
\begin{equation}
	\hspace*{-20pt}
	\begin{aligned}
		N_{i}(n) = & \sum_{t=1}^{n} \mathbb{I}\left\{A_{t}=i\right\}                                                                                                                                                                                                                                                                                          \\
		\leq       & \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\}}_{\text{(A)}}+ \underbrace{\sum_{t=1}^{n} \mathbb{I}\left\{\hat{\mu}_{i}(t)+\sqrt{\frac{2 \log t}{\widetilde{N}_i(t)}} \geq \mu_{1}-\varepsilon \text { and } A_{t}=i\right\}}_{\text{(B)}} \\
	\end{aligned}
\end{equation}
\normalsize

Given $\widetilde{N}_i(t) \ge N_i(t)$, we can relax (B) by replacing
$\widetilde{N}_i(t)$ with $N_i(t)$, which makes it identical to the case of UCB
and automatically arrive to $1 + \frac{2(\log t+\sqrt{\pi \log
	t}+1)}{\left(\Delta_{i}-\varepsilon\right)^{2}}$ according to
\citep{lattimore2020bandit}. At the same time, we have $\widetilde{N}_i(t) \le
t$, but we cannot apply a similar procedure to (A) because directly replacing
$\widetilde{N}_i(t)$ with $t$ will make (A) grow much faster and violate the
\textit{sub-UCB} condition.

%, which we show in appendix \ref{apn:need_for_explore_as}.

\begin{assumption}
	There exists time step $\tau$, which ensures the policy chooses $A_1$ often
	enough:
	\vspace{-0.5em}
																																																																																																																																																																																																							
	$$
	\tau=\min \left\{t \leq T: \sup _{s \geq t}\left|\hat{\mu}_{1}(s)-\mu_{1}\right|<\varepsilon\right\}
	$$

	\vspace{-0.5em}
																																																																																																																																																																																																							
	\label{assumption:enough}
\end{assumption}

If we can leverage assumption \ref{assumption:enough}, then a simple observation
is that:


\begin{equation}
	\begin{aligned}
		\sum_{t=1}^{T} \mathbb{I}\left\{\hat{\mu}_{1}(t)+\sqrt{\frac{2 \log (t) }{\widetilde{N}_1(t)}}  \leq \mu_{1}-\varepsilon\right\} &   
		\le  \tau + \sum_{t=\tau+1}^T \mathbb{I}\{ \mu_1 - \hat{\mu}_1(t) \ge \varepsilon + \delta \}
	\end{aligned}
\end{equation}

It is straightforward to see that $P( \mu_1 - \hat{\mu}_1(t) \ge \varepsilon +
\delta \mid t > \tau) = 0$, where $\sqrt{2\log(t) / t}$ is replaced with $\delta
> 0$. Therefore, the (A) can be bounded within $\tau$. Furthermore, if we let
bandit distribution to be gaussian, then by the concentration Lemma 1 in
\citep{lattimore2018refining}, $\mathbb{E}[\tau] \le 1+9 / \varepsilon^{2}$. Thus
the regret of UCB-DT is clearly upper bounded with \textit{sub-UCB} requirement.


Take UCB-DT($\mu$) as an example, we can reach the assumption
\ref{assumption:enough} as long as $\gamma$ to be small enough, such as $1 /
N_{bargain}$ according to Sec.~\ref{sec:bargain_point}. In fact, UCB-DT
can represent a family of policies through parameterization of $d$, and the
regret bound here only describes the boundary behavior as it approaches the vanilla UCB.
Based on our previous analysis,
there exists a parameter space of $d$ which can be used to customize towards better
exploration-exploitation trade-off. Therefore, instead of diving into a detailed
regret expression of any specific form, we provide a general analysis without
explicitly including the degree of freedom.


\section{Numerical Experiments}
\label{sec:exp}

We compare UCB-DT to UCB \citep{auer2002finite}, UCB$\dagger$
\citep{lattimore2018refining}, UCBV-Tune \citep{audibert2009exploration}, KL-UCB
\citep{garivier2011kl, cappe2013kullback} and KL-UCB++ \citep{menard2017minimax}.
Among these methods, UCB, UCB$\dagger$ and UCBV-Tune are our main comparisons,
though UCB-DT can also be readily extended to support variance adaption.
The remaining two methods, KL-UCB and KL-UCB++,  which delivers excellent
performance, are \textit{non-anytime} policies. Because of these structural
differences, we do not regard them as our main comparisons, but we still keep
them as important references.




\begin{table}[h]
	\centering
	\begin{tabular}{lrrrrrr}
		\hline
		Experiment      & KL-UCB & KL-UCB++        & UCBV-Tune & UCB$\dagger$ & UCB     & UCB-DT($\mu$)  \\
		\hline
		B5 *            & 41.73  & \textbf{38.03}  & 98.6      & 129.01       & 251.28  & 70.95          \\
		B20 *           & 168.54 & \textbf{129.5}  & 415.23    & 410.5        & 939.99  & 383.82         \\
		B(0.02, 0.01) * & 28.34  & 22.39           & 64.99     & 131.99       & 249.17  & \textbf{21.6}  \\
		B(0.9, 0.88) *  & 38.44  & 33.78           & 49.6      & 73.9         & 119.91  & \textbf{19.19} \\
		N5 *            & 194.82 & 109.75          & 119.97    & 88.3         & 142.21  & \textbf{83.65} \\
		N20             & 539.91 & \textbf{410.25} & 840.26    & 560.47       & 1014.27 & 640.52         \\
		\hline
	\end{tabular}
	\vspace*{2pt}
	\caption{Regret of different policies in each environment.
		For each environment, we mark bold text for the best result and "*" if
		UCB-DT outperforms UCB, UCB$\dagger$ and UCBV-Tune.}
	\label{tab:regret}
\end{table}

For thorough experimentation, we design 6 environments as below

\begin{description}[leftmargin=!,labelwidth=\widthof{\bfseries B(0.02, 0.01)}]
	\item[B5] Bernoulli reward, 5 bandits with expected rewards 0.9, 0.8, 0.7, 0.2,
	0.5. This environment is modified from \citep{garivier2011kl} by adding more bandits.
	\item[B20] Bernoulli reward with many bandits, 20 bandits with expected rewards 0.9, 0.85, 0.8, 0.8, 0.7,
	0.65, 0.6, 0.6, 0.55, 0.5,
	0.4, 0.4, 0.35, 0.3, 0.3,
	0.25, 0.2, 0.15, 0.1, 0.05.
	\item[B(0.02, 0.01)] Bernoulli reward with low means, 3 bandits with expected rewards 0.05,
	0.02, 0.01. This environment is borrowed
	identically from \citep{garivier2011kl}.
	\item[B(0.9, 0.88)] Bernoulli reward with close means, 2 bandits with expected rewards 0.9,
	0.88. 
	\item[N5] Gaussian reward, 5 bandits with unit variance and expected rewards
	1, 0.8, 0.5, 0.3, -0.2.
	\item[N20] Gaussian reward with many bandits, 20 bandits with unit variance and expected rewards
	0, -0.03, -0.03, -0.07, -0.07, -0.07, -0.15, -0.15, -0.15, -0.5, -0.5, -0.5,
	-0.5, -0.5, -0.5, -0.5, -0.5, -0.5, -1, -1. This environment is borrow identically
	from \citep{lattimore2018refining}.
\end{description}



We set $T$ to 20000 and run 2000 simulations for each method on every
environment. We do not specifically adjust the speed parameter, and we set
$\gamma$ to 0.02 in all experiments. For other methods, we use implementations
and default parameters from \citep{SMPyBandits}. We summarize cumulative regrets
in table \ref{tab:regret} and Fig. \ref{fig:exp}.

From experiment results, we can see that UCB-DT is always better than UCB and
outperforms UCB$\dagger$, UCBV-Tune in 5 environments. We speculate the reason
of smaller improvement margin in N20 comes from the high variance of the 
environment, which makes the estimation of distance unstable. This behavior can
be alleviated with different distance designs as in Appendix \ref{apn:more_d}.

% \section{Related Work}

\section{Conclusion}

By leveraging bandit distance, we create a policy called UCB-DT, which is
simple, extensible and performant. With analysis of our policy, we propose
the concept of \textit{Exploration Bargain Point} to provide a new perspective
on analyzing performance of UCB-based methods.
Admittedly, this work bears its own limitations. We did not dive deeper in the
regret bound analysis to describe relationship between convergence behavior and
possible properties of $d$. We only study the \textit{Exploration Bargain Point}
in the context of our method and standard UCB but haven't applied it to other
UCB-based policies.
However, we believe these limitations could be regarded as future possibilities
in this direction, and it is also possibly promising to adopt the idea in this paper to
more general settings like adversarial bandit and reinforcement learning.



==> include.backup1004/preamble.tex <==
\usepackage{xcolor}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks [hidelinks]
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{algorithmic}
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{wrapfig}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage[boxruled]{algorithm2e}
\usepackage{enumitem}
\usepackage{float}

\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}

\usepackage{bbm}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{scalerel}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand\tocite[1]{\textcolor{red}{[#1]}}
\newcommand\tosupple[1]{\textcolor{red}{[supplement #1]}}
\newcommand\mshift[1]{\hat{\mu}_{\Delta_{#1}}}

\newtheorem{assumption}{Assumption}
\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


%% This part goes in preamble
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


\newcommand{\quotes}[1]{``#1''}


\definecolor{YellowOrange}{RGB}{247, 146, 28}
\definecolor{NavyBlue}{RGB}{2, 110, 184}
\definecolor{DarkGreen}{RGB}{85, 168, 104}
\definecolor{DarkRed}{RGB}{196, 78, 82}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

